ChatGPT in the Classroom: An Analysis of Its Strengths and Weaknesses for Solving Undergraduate Computer Science Questions

ChatGPT is an AI language model developed by OpenAI that can understand and generate human-like text. It can be used for a variety of use cases such as language generation, question answering, text summarization, chatbot development, language translation, sentiment analysis, content creation, personalization, text completion, and storytelling. While ChatGPT has garnered significant positive attention, it has also generated a sense of apprehension and uncertainty in academic circles. There is concern that students may leverage ChatGPT to complete take-home assignments and exams and obtain favorable grades without genuinely acquiring knowledge. This paper adopts a quantitative approach to demonstrate ChatGPT's high degree of unreliability in answering a diverse range of questions pertaining to topics in undergraduate computer science. Our analysis shows that students may risk self-sabotage by blindly depending on ChatGPT to complete assignments and exams. We build upon this analysis to provide constructive recommendations to both students and instructors.

==> sections/04-results.tex <==
% \begin{itemize}
%     \item {\color{red} High level summary - number of questions, how many of them are correct, incorrect, partially correct - we can probably have a table summarizing all the undergrad courses, GATE and LeetCode }
%     \item {\color{red} Can we categorize the questions into multiple sub-categories: objective type, single word, descriptive, numericals etc.}
%     \item Add graphs or any other visualization. 
% \end{itemize}
% \renewcommand{\arraystretch}{1.1}

% \begin{table*}[!ht]
%     \centering
%     \resizebox{0.9\textwidth}{!}{%
%     \begin{tabular}{|c|c|l|}
%         \hline
%         \textbf{Subject} & \textbf{Accuracy} & \textbf{Description} \\
%         \hline
%         \multirow{2}{*}{\hfil \textbf{GATE}} & \multirow{2}{*}{\hfil \(49\%\)} & 49 Correct (\textit{34 numerical, 16 theory, 1 coding}) \\
%         & & 51 Incorrect (\textit{32 numerical, 19 theory})  \\
%         \hline
%         \multirow{3}{*}{\hfil \textbf{Operating Systems}} & \multirow{3}{*}{\hfil \(58.41\%\)} & 59 Correct (\textit{15 T/F, 27 theory, 5 design, 5 coding, 8 Numerical}) \\
%         & & \parbox{28em}{17 Partially Correct 
%         (\textit{1 T/F, 1 theory, 0 design, 6 coding, 9 Numerical})}\\
%         & & 25 Incorrect 
%         (\textit{4 T/F, 4 theory, 0 design, 5 coding, 12 Numerical})\\
%         \hline
%         \multirow{3}{*}{\textbf{\parbox{7em}{\centering Data Structure and Algorithms}}} & \multirow{3}{*}{\hfil \(70.01\%\)} & 75 Correct (\textit{32 T/F, 15 theory, 14 design, 10 coding, 4 Numerical}) \\
%         & & \parbox{28em}{14 Partially Correct (\textit{3 T/F, 6 theory, 2 design, 0 coding, 3 Numerical})}\\
%         & & 18 Incorrect (\textit{5 T/F, 7 theory, 4 design, 1 coding, 1 Numerical})\\
%         \hline
%         \multirow{4}{*}{\hfil \textbf{LeetCode Coding}} & \multirow{2}{*}{\hfil \textbf{Cat.I}: \(53.06\%\)} & 26 Accepted (\textit{All test cases passed}) \\
%         & & 23 Partially Accepted (\textit{\(\geq1\) test cases passed}) \\\cline{2-3}
%         & \multirow{2}{6.75em}{\hfil \textbf{Cat.II}: \(94.2\%\)} & 65 Accepted (\textit{All test cases passed}) \\
%         & & 4 Partially Accepted (\textit{\(\geq1\) test cases passed}) \\
%         \hline
%         \multirow{4}{*}{\hfil \textbf{Machine Learning}} & \multirow{4}{*}{\hfil \(51.35\%\)} & 57 Correct (\textit{16 MSQs, 41 theory}) \\
%         & & 5 Partially correct (5 theory) \\
%         & & 43 Incorrect (\textit{34 MSQ, 9 theory})\\
%         & & 6 Not solvable through ChatGPT (\textit{2 MSQ, 4 theory}) \\
%         \hline
%         \multirow{4}{12em}{\hfil \textbf{\parbox{10em}{\centering Database Management Systems}}} & \multirow{4}{*}{\hfil \(33.33\%\)} & 36 Correct (\textit{9 MSQs, 27 theory}) \\
%         & & 15 Partially correct (4 MSQ, 11 theory) \\
%         & & 55 Incorrect (\textit{14 MSQ, 41 theory})\\
%         & & 2 Not solvable through ChatGPT (\textit{2 theory}) \\
%         \hline
%     \end{tabular}}
%     \caption{Analysis of ChatGPT's performance in undergraduate computer science subjects}
%     \label{tab:results}
% \end{table*} 
% \renewcommand{\arraystretch}{1}

Figure \ref{fig:dsa} gives an overview of ChatGPT's performance on the collected data. We discuss the details next:
% \begin{figure*}[!ht]
\begin{figure*}[ht]
      \includegraphics[width=0.97\textwidth]{sections/images/paper_figure_final_300-01.png}
      \caption{ChatGPT performance on \textit{(clockwise from top-left)}: Data Structures and Algorithms, Operating Systems, Database Management Systems, Leetcode, GATE, Machine Learning}
      \label{fig:dsa}
      \vspace{-1em}
\end{figure*}

% \subsubsection{\color{red}Undergraduate computer science subjects:}
% \subsubsection{Undergraduate computer science subjects:}
\subsection{Undergraduate computer science subjects:}

\subsubsection{\textbf{Data Structures and Algorithms:}}
    Out of the 107 questions on DSA used to evaluate ChatGPT, it provided correct responses for 75 questions, incorrect responses for 18 questions, and partially correct responses for the remaining 14 questions. The fraction of the correct answers was different for different types of questions. ChatGPT was able to give correct responses for 32 out of 40 true/false questions, 15 out of 28 short/long answer questions, 14 out of 20 design-based questions, and 10 out of 11 coding related questions. It is interesting to note that ChatGPT sometimes answers very basic questions incorrectly, even if they can be solved by a simple formula. On the other hand, it gives very well framed answers for more difficult questions. An example of a basic question answered incorrectly is:
    
\noindent \textbf{\small State True or False: Given a directed graph G = (V, E), run breadth-first search from a vertex $s \in V$ . While processing a vertex u, if some $v \in Adj+(u)$ has already been processed, then G contains a directed cycle.}
    
    % Refer to Fig. \ref{fig:dsa}.
    % \begin{figure}[!ht]
    %   \centering
    %   \includegraphics[width=0.33\textwidth]{sections/images/dsa.png}
    %   \caption{ChatGPT performance on Data Structure and Algorithms questions}
    %   \label{fig:dsa}
    % \end{figure}

\subsubsection{\textbf{Operating Systems:}} 
    Out of the 101 questions on OS used to evaluate ChatGPT, 59 were answered correctly, 25 were answered incorrectly, and 17 were answered partially correct by ChatGPT. The nature of the correct answers varied, with 15 out of 20 true or false questions being answered correctly and justified, 27 out of 32 short/long answer questions being answered correctly, 5 out of 5 design-based questions being answered correctly, and only 4 out of 15 coding-related questions being answered correctly. Directly asking questions without laying down the context tends to be a reason for lower accuracy, and leads to ChatGPT fixating on wrong parts of the question. An example of a question answered wrongly by ChatGPT and then answered correctly with context is:
    
    \noindent \textbf{\small What is the value of x at the end of this code? Assume that 3pixels.jpg has 3 pixels. Show your work for partial credit. x = 3; y = 7; img = new SimpleImage("3pixels.jpg"); for (pixel : img) \{ x = x + y; x = x + 1; y = 1; \} }
    % Refer to Fig. \ref{fig:os}.
    % \begin{figure}[!ht]
    %   \centering
    %   \includegraphics[width=0.33\textwidth]{sections/images/os.png}
    %   \caption{ChatGPT performance on Operating Systems questions}
    %   \label{fig:os}
    % \end{figure}

\subsubsection{\textbf{Database Management System:}}
    Out of the 108 questions on DBMS used to evaluate ChatGPT, it was able to answer 36 questions correctly, 55 questions incorrectly, and 15 questions partially correct. There were two questions that ChatGPT was unable to process. The questions were divided into two categories: MSQ and theory questions. ChatGPT correctly answered 9 out of 27 MSQs and 27 out of 81 theory questions. It gave partially correct responses to 4 MSQs and 11 theory questions. Rest were all incorrectly answered by ChatGPT.
    % There were no MSQ questions that ChatGPT was unable to answer, but there were two theory questions that ChatGPT was unable to process.
    We observed similar behaviour of ChatGPT when it comes to answering simple questions incorrectly and complex questions correctly, as in the case of DSA and OS.
    % Refer to Fig. \ref{fig:dbms}.
    % \begin{figure}[!ht]
    %   \centering
    %   \includegraphics[width=0.33\textwidth]{sections/images/dbms.png}
    %   \caption{ChatGPT performance on DBMS questions}
    %   \label{fig:dbms}
    % \end{figure}

\subsubsection{\textbf{Machine Learning:}}
     The study evaluated ChatGPT's performance on machine learning questions, consisting of 52 MSQ and 59 theory questions. For MSQ, ChatGPT answered 16 questions correctly and 34 questions incorrectly. For theory questions, ChatGPT answered 41 questions correctly, 9 questions incorrectly, and 5 questions partially correct. However, there were 4 theory questions and 2 MSQs that ChatGPT was unable to process. Overall, the study consisted of 111 questions, and ChatGPT's performance was not very accurate, particularly for MSQs, where it answered less than one-third of the questions correctly. ChatGPT apologises in case we provide more information about the question after it has given an answer, and discards the previous details to give an incorrect answer. Solving basic mathematical problems was difficult for ChatGPT, rendering it to be not so helpful in the case of an aptitude based ML problem. For example: 
    
    \noindent \textbf{\small When asked to compute the determinant of the matrix A = [[22/5, -6/5], [-6/5, 13/5]], ChatGPT gave the wrong answer det(A)  = 322/25 while the correct answer is 10.}
    % Refer to Fig. \ref{fig:ml}.
    % \begin{figure}[!ht]
    %   \centering
    %   \includegraphics[width=0.33\textwidth]{sections/images/ml.png}
    %   \caption{ChatGPT performance on Machine Learning questions}
    %   \label{fig:ml}
    % \end{figure}

% \begin{itemize}
%     \item \textbf{Data Structures and Algorithm: } 
%     In the testing of ChatGPT's performance on data structures and algorithm questions, a total of 107 questions were evaluated. The results showed that ChatGPT provided correct responses for 75 questions, incorrect responses for 18 questions, and partially correct responses for 14 questions. The nature of the correct answers varied, with 32 out of 40 questions that required a true or false response being answered correctly and justified, 15 out of 28 short/long answer questions being answered correctly, 14 out of 20 design-based questions being answered correctly, and 10 out of 11 coding related questions being answered correctly. Refer to Fig. \ref{fig:dsa}.
%     \begin{figure}[!ht]
%       \centering
%       \includegraphics[width=0.4\textwidth]{sections/images/dsa.png}
%       \caption{ChatGPT performance on Data Structure and Algorithms questions}
%       \label{fig:dsa}
%     \end{figure}


%     \item \textbf{Operating Systems: } 
%     In the study evaluating ChatGPT's performance on operating system questions, a total of 101 questions were asked. Out of these, 59 were answered correctly, 25 were answered incorrectly, and 17 were partially correct. The nature of the correct answers varied, with 15 out of 20 true or false questions being answered correctly and justified, 27 out of 32 short/long answer questions being answered correctly, 5 out of 5 design-based questions being answered correctly, and only 4 out of 15 coding-related questions being answered correctly. Refer to Fig. \ref{fig:os}.
%     \begin{figure}[!ht]
%       \centering
%       \includegraphics[width=0.4\textwidth]{sections/images/os.png}
%       \caption{ChatGPT performance on Operating Systems questions}
%       \label{fig:os}
%     \end{figure}

%     \item \textbf{Database Management System: }
%     The study tested ChatGPT's performance on Database Management System questions, with a total of 108 questions. Out of these, ChatGPT was able to answer 36 questions correctly, 55 questions incorrectly, and 15 questions partially correct. There were two questions that ChatGPT was unable to process. The questions were divided into two categories: Multiple Select questions (MSQ) and theory questions. ChatGPT correctly answered 9 out of 27 MSQs and 27 out of 81 theory questions. It gave incorrect responses to 14 MSQs and 41 theory questions. For MSQs, ChatGPT partially answered 4 questions correctly out of 27, and for theory questions, ChatGPT was able to partially answer 11 questions correctly out of 81. There were no MSQ questions that ChatGPT was unable to answer, but there were two theory questions that ChatGPT was unable to process. Refer to Fig. \ref{fig:dbms}.
%     \begin{figure}[!ht]
%       \centering
%       \includegraphics[width=0.4\textwidth]{sections/images/dbms.png}
%       \caption{ChatGPT performance on DBMS questions}
%       \label{fig:dbms}
%     \end{figure}

%     \item \textbf{Machine Learning: }
%     The study evaluated ChatGPT's performance on machine learning questions, consisting of 52 Multiple Select questions (MSQ) and 59 theory questions. For MSQ, ChatGPT answered 16 questions correctly and 34 questions incorrectly. For theory questions, ChatGPT answered 41 questions correctly, 9 questions incorrectly, and 5 questions partially correct. However, there were 4 theory questions and 2 MSQs that ChatGPT was unable to solve. Overall, the study consisted of 111 questions, and ChatGPT's performance was not very accurate, particularly for MSQs, where it answered less than one-third of the questions correctly. Refer to Fig. \ref{fig:ml}.
%     \begin{figure}[!ht]
%       \centering
%       \includegraphics[width=0.4\textwidth]{sections/images/ml.png}
%       \caption{ChatGPT performance on Machine Learning questions}
%       \label{fig:ml}
%     \end{figure}
    
% \end{itemize}

% \subsubsection{Graduate Aptitude Test in Engineering (GATE)}
\subsection{Graduate Aptitude Test in Engineering (GATE)}
Out of the 100 GATE questions used to evaluate ChatGPT, 49 questions were answered correctly by ChatGPT, while 51 questions were incorrect.
Out of the 51 incorrect answers, 32 were numerical questions. Among the numerical questions, 3 questions were related to coding, and 2 questions required both theory and numerical comprehension. The remaining 19 incorrect answers were related to theory questions.
Among the 49 correct answers provided by ChatGPT, 34 were related to numerical questions, and 2 of these numerical questions required coding. Additionally, 16 correct answers were related to theory questions, and 2 of these required coding. Lastly, there was 1 correct answer related to coding.
Overall, out of the 100 questions tested, there were 35 theory questions and 69 numerical questions. In majority of the incorrect answers, ChatGPT has provided the correct explanation and reached the correct answers but failed to select the option corresponding to the correct answer as the final output.
% Refer to Fig. \ref{fig:gate}.
% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.33\textwidth]{sections/images/gate.png}
%   \caption{ChatGPT performance on GATE questions}
%   \label{fig:gate}
% \end{figure}

% Based on the given statistics, ChatGPT's performance on answering GATE questions is not ideal. The fact that it could only answer 49 out of 100 questions correctly implies that its performance is below average. Additionally, the majority of the incorrect answers were for numerical questions, which suggests that ChatGPT might not be well-equipped to answer numerical questions accurately. However, it did perform relatively better on theory and coding questions.

% While it is difficult to draw definitive conclusions about ChatGPT's overall capabilities based on just one test, these statistics suggest that there is room for improvement in its ability to answer GATE questions, particularly in the numerical domain.

% If a student is relying solely on ChatGPT to prepare for their GATE examination, the given statistics should serve as a warning that it may not be a reliable source of answers for all types of questions. In particular, the fact that it struggled with numerical questions could potentially be a cause for concern, as these types of questions often carry a significant weightage in GATE exams.

% \subsubsection{Programming questions from LeetCode}
\subsection{Programming questions from LeetCode}
LeetCode questions used for evaluating ChatGPT were divided into two categories. Category 1 involved direct questions from LeetCode, while category 2 included frequently asked technical interview questions by top technology companies. 
For questions in Category 2, ChatGPT was given the following context before being prompted with the actual question: \textit{"You are computer science UG student preparing for technical interviews. Please answer the below questions"}.
ChatGPT was able to provide correct code for almost all questions in category 2, along with answering follow-up questions such as the time complexity of the code. Surprisingly, in all the questions in category 2, ChatGPT generated the same function name as provided in LeetCode. 
% All 65 questions in category 2 were accepted in one go, and none were unable to answer.

On the other hand, questions in category 1 were directly fed to ChatGPT without any prior prompt. There was no recognizable pattern regarding the questions ChatGPT could answer correctly, as it could fail for easy questions and pass hard ones with flying colors. ChatGPT generated code that passed at least one test case, if not all the test cases. The solutions given by ChatGPT were categorized into two buckets: accepted (all test cases passed) and partial correct (one or more test cases passed, but not all). Out of the \textcolor{red}{48 questions in category 1, 26 were accepted, and 23 were partial correct.} 
% Refer to Fig. \ref{fig:leetcode_c1}.

Overall, ChatGPT was able to generate correct code for most category 2 questions and showed a varying performance for category 1 questions. The study suggests that providing a prompt before presenting the questions to ChatGPT could improve its performance in generating correct code. 
% Refer to Fig. \ref{fig:leetcode_c2}.

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.33\textwidth]{sections/images/leetcode_c1.png}
%   \caption{ChatGPT performance on LeetCode (Cat. I) questions}
%   \label{fig:leetcode_c1}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.33\textwidth]{sections/images/leetcode_c2.png}
%   \caption{ChatGPT performance on LeetCode (Cat. II) questions}
%   \label{fig:leetcode_c2}
% \end{figure}

